A Multi-Modal Approach to Infer Image Affect

The group affect or emotion in an image of people can be inferred by extracting features about both the people in the picture and the overall makeup of the scene. The state-of-the-art on this problem investigates a combination of facial features, scene extraction and even audio tonality. This paper combines three additional modalities, namely, human pose, text-based tagging and CNN extracted features / predictions. To the best of our knowledge, this is the first time all of the modalities were extracted using deep neural networks. We evaluate the performance of our approach against baselines and identify insights throughout this paper.

==> Feature_Fusion.tex <==
\section{Feature Aggregation}

As previously discussed in Section ~\ref{sec:sec3}, given a group level image, our methodology consists of extracting scene related features using CENTRIST, facial features using RESNET, human pose features using a pre-trained NN and BOW descriptors using the im2txt neural network. In this section, we describe our strategy for combining features extracted from all the group level images to build the training data for classification. 

Our feature combination strategy involves concatenating all the features for each group level image. It is important to note that, in this problem of group level emotion recognition, feature concatenation is not straight-forward. The feature vectors extracted from CENTRIST and the bag-of-words extracted from the im2txt NN are already on a per image basis.However, this is not the case for the facial and pose features since these features are extracted for each human in the images and need to be aggregated across all the humans for each group level image, before concatenation.

We adopt a bag-of-visual-words (BOV) based approach to construct image level aggregated feature vectors using the facial and pose features for each group level image evaluated using the methods described in Section and Section. The BOV based feature transformation is carried out separately for both facial and pose features. 

In our BOV based approach, the feature vector corresponding to each face or pose, is regarded a visual word as a result of which the number of visual words is equal to the total number of humans extracted over all the group level images. Having defined the visual word, the BOV based feature aggregation is described as follows.
\begin{enumerate}
\item \underline{k-means Based Methodology}
The set of visual words is clustered using the k-means algorithm to reduce the vocabulary which consists of the cluster labels, also referred to as visual codes. From clusters resulting from the k-means clustering algorithm, we develop three group level feature vectors as follows. 

\begin{enumerate}
\item	A term frequency (TF) matrix which consists of the associating each face in the group level image to a visual code and the counting the occurrence of each visual code in the vocabulary. The values are also normalized by dividing each count by the total number of faces (visual words) in the image. Denoting the raw count of a visual code $l$ for a given image $m$ as $t_{l,m}$, the TF is simply given as,
\begin{equation}
tf(i,m) = \frac{ t_{l,m}} {\sum_{l^{\prime} \in m} t_{l^ {\prime},m}}
\end{equation}

\item The second feature, that we evaluate using the cluster center is the vector of locally aggregated descriptors (VLAD). VLAD is a feature encoding method that takes into account the strength of association of each visual word to its cluster center. 

Defining the strength of association of each visual word ${w_i}$ ($i=1,\ldots,n$) to cluster $k$ as $q_{ik}$, where $q_{ik} \geq 0$ and $\sum_{i=1}^{n} q_{ik} = 1$, the VLAD encoding using the cluster centroids $\mu_{k}$ is defined as,

\begin{equation}
v_k = \sum_{i=1}^{n} q_{ik} (w_{ik} - \mu_k)
\end{equation}

The primary advantage of VLAD over the TF matrix is that more discriminative property is added in our feature vector by taking the difference of each descriptor from the mean in its voronoi cell. This first order statistic adds more information in the feature vector and may give us better discrimination during classification. The VLAD encodings are usually normalized (e.g. $l^2$ normalization) before usage.
	
\item The third feature vector, resulting from the k-means clustering algorithm is a weighted average (WA) of the cluster centers for each visual word in the image. The  weights are nothing but the normalized term frequencies corresponding to each visual word.
\end{enumerate}

\item \underline{GMM Based Methodology}  In addition to the k-means clustering method, we also perform a dimensionality reduction of the visual codes using GMM. The aggregation  involves computing the posterior probability of each component for a given visual word, which is also defined as the responsibility that a particular component takes in explaining that visual word. The responsibilities of a given component resulting from all the faces in a given image are averaged to compute the group level image responsibility for that component. Performing the same computation for all the components using the visual words in a given image results in an image level aggregated feature vector.

\end{enumerate}

It can be noted that all the four feature vectors described above, namely, the TF matrix, VLAD, the weighted average of the cluster centers and the GMM based features have dimensions $N \times K$, where $K$ is either the number of clusters for the k-means algorithm or the number of Gaussians for the GMM model. Since all the features are now consistent in terms of their dimensions and are group-image level features, they can be easily concatenated. The series of above described steps are carried out for both the training and the validation image sets to construct the features for classification.



\subsubsection{Auto-Regression Decoding}
